MIG-COW: Transferable Adversarial Attacks on Deepfake Detectors via Gradient Decomposition

Despite recent advances, deepfake detectors remain vulnerable to adversarial examples, particularly in diverse, real-world settings. We propose MIG-COW, a novel adversarial attack framework that generates highly generalizable and visually imperceptible adversarial examples. By combining momentum-integrated gradients with a consensus-orthogonal decomposition, MIG-COW captures both shared and model-specific vulnerabilities across heterogeneous CNN and ViT detectors. On the AADD-2025 Challenge benchmarks, MIG-COW achieves a 99.96% white-box attack success rate (ASR) with high perceptual similarity (SSIM), significantly outperforming existing baselines. However, its limited 7.16% ASR against official black-box targets - despite achieving the best overall score - highlights the ongoing challenge of transferability. We also demonstrate that incorporating low-performing but diverse models in the ensemble can degrade attack effectiveness, underscoring the need for careful surrogate model selection in real-world adversarial settings.

==> mathsymbol.tex <==
% Number Sets
\newcommand{\N}{\mathbb{N}\xspace}
\newcommand{\Z}{\mathbb{Z}\xspace}
\newcommand{\Q}{\mathbb{Q}\xspace}
\newcommand{\R}{\mathbb{R}\xspace}
\newcommand{\C}{\mathbb{C}\xspace}
\newcommand{\sI}{\mathbb{I}\xspace}

% Special Sets
\newcommand{\B}{\mathcal{B}\xspace}
\newcommand{\D}{\mathcal{D}\xspace}
\newcommand{\V}{\mathcal{V}\xspace}
\newcommand{\RR}{\mathcal{R}\xspace}
\newcommand{\SSS}{\mathcal{S}\xspace}
\newcommand{\sV}{\mathcal{V}\xspace}

% scheme elts
\newcommand{\CKKS}{CKKS\xspace}
\newcommand{\Setup}{\textsf{Setup}\xspace}
\newcommand{\KeyGen}{\textsf{KeyGen}\xspace}
\newcommand{\Rot}{\textsf{Rot}\xspace}

\newcommand{\Message}{Message\xspace}
\newcommand{\Encode}{\textsf{Ecd}\xspace}
\newcommand{\Decode}{\textsf{Dcd}\xspace}
\newcommand{\Encrypt}{\textsf{Enc}\xspace}
\newcommand{\Decrypt}{\textsf{Dec}\xspace}
\newcommand{\DecryptApprox}{\textsf{DecryptApprox}\xspace}
\newcommand{\Verify}{\textsf{Verify}\xspace}
\newcommand{\Evaluate}{\textsf{Evaluate}\xspace}
\newcommand{\Ecdtype}{\textsf{EcdType}\xspace}
\newcommand{\Boot}{\textsf{Boot}\xspace}
\newcommand{\Inv}{\textsf{Inv}\xspace}
\newcommand{\Prec}{\textsf{PrecLoss}\xspace}
\newcommand{\Cleanse}{\textsf{Cleanse}\xspace}
\newcommand{\SqMethod}{\textsf{SqMethod}\xspace}
\newcommand{\paramsq}{\textsf{paramSq}\xspace}
\newcommand{\paramind}{\textsf{paramInd}\xspace}

\newcommand{\Reord}{\textsf{ReOrd}\xspace}
\newcommand{\Rankvec}{\textsf{RankVec}\xspace}
\newcommand{\Ranksort}{\textsf{RankSelect}\xspace}
\newcommand{\Privtopk}{\textsf{PrivTopk}\xspace}
\newcommand{\PrivMT}{\textsf{PrivTopk}_{MT}\xspace}

\newcommand{\Blocktopk}{\textsf{BlockTopk}\xspace}
\newcommand{\BlocktopkS}{\textsf{BlockTopk}_S\xspace}
\newcommand{\BlocktopkM}{\textsf{BlockTopk}_M\xspace}
\newcommand{\BlocktopkMT}{\textsf{BlockTopk}_{MT}\xspace}
\newcommand{\Merge}{\textsf{Merge}\xspace}
\newcommand{\Mergeone}{\textsf{MergeToOne}\xspace}
\newcommand{\Itermax}{\textsf{IterMax}\xspace}



\newcommand{\al}{\textsf{Algo}\xspace}
\newcommand{\sinc}{\textsf{Sinc}\xspace}
\newcommand{\argmax}{\textsf{argmax}\xspace}
\newcommand{\argmin}{\textsf{argmin}\xspace}

\newcommand{\summation}{\textsf{Sum}\xspace}
\newcommand{\rotsum}{\textsf{RotSum}\xspace}
\newcommand{\spread}{\textsf{Spread}\xspace}
\newcommand{\rowsum}{\textsf{RowSum}\xspace}
\newcommand{\colsum}{\textsf{ColSum}\xspace}
% \newcommand{\copyr}{\textsf{RowSpread}\xspace}
% \newcommand{\copyc}{\textsf{ColSpread}\xspace}
\newcommand{\copyr}{\textsf{RowCopy}\xspace}
\newcommand{\copyc}{\textsf{ColCopy}\xspace}
\newcommand{\rowtrans}{\textsf{RowTrans}\xspace}
\newcommand{\coltrans}{\textsf{ColTrans}\xspace}



% functions
\newcommand{\Add}{\textsf{Add}\xspace}
\newcommand{\Mult}{\textsf{Mult}\xspace}
\newcommand{\Rescale}{\textsf{Rescale}\xspace}


\newcommand{\pk}{\Vec{pk}\xspace}
\newcommand{\sk}{\Vec{sk}\xspace}
\newcommand{\rk}{\Vec{rk}\xspace}

\newcommand{\m}{{m}\xspace}
\newcommand{\evk}{\Vec{evk}\xspace}
\newcommand{\pt}{\textit{pt}\xspace}
\newcommand{\ct}{\Vec{ct}\xspace}
% \newcommand{\res}{\Vec{r}\xspace}
\newcommand{\basis}{\Vec{b}\xspace}
\newcommand{\fullbasis}{\Vec{fb}\xspace}

\newcommand{\ohebasis}{\Vec{B}\xspace}
\newcommand{\CT}{\Vec{C}\xspace}
\newcommand{\rc}{\Vec{ct}_{rc}\xspace}
\newcommand{\cc}{\Vec{ct}_{cc}\xspace}
\newcommand{\cci}{\Vec{ct}_{cc,i}\xspace}
\newcommand{\cck}{\Vec{ct}_{cc,k}\xspace}
\newcommand{\res}{\Vec{ct}_{out}\xspace}
\newcommand{\ress}{\Vec{ct}_{out,s}\xspace}
\newcommand{\rest}{\Vec{ct}_{out,t}\xspace}
\newcommand{\resi}{\Vec{ct}_{out,i}\xspace}
\newcommand{\resj}{\Vec{ct}_{out,j}\xspace}


\newcommand{\ind}{\textsf{ind}\xspace}
\newcommand{\Eqtest}{\textsf{eqtest}\xspace}

\newcommand{\TF}{\textsf{TF}\xspace}
\newcommand{\BoW}{{BoW}\xspace}
\newcommand{\Dist}{\textsf{Distance}\xspace}
\newcommand{\Comp}{\textsf{Comp}_p\xspace}
\newcommand{\Compn}{\textsf{Comp}_p^q\xspace}
\newcommand{\comp}{\textsf{comp}\xspace}
\newcommand{\sign}{\textsf{sign}\xspace}
\newcommand{\Sign}{\textsf{Sign}\xspace}
\newcommand{\ESF}{\textsf{ESF}\xspace}
\newcommand{\Max}{\textsf{Max}\xspace}

\newcommand{\topk}{Top-$k$\xspace}
\newcommand{\knn}{$k$-NN\xspace}


\newcommand{\Count}{\textsf{Count}\xspace}
\newcommand{\NaiveCount}{\textsf{NaiveCount}\xspace}
\newcommand{\Numof}{\textsf{Numof}\xspace}
\newcommand{\CountEB}{\textsf{CountEB}\xspace}



\newcommand{\DF}{\textsf{DF}\xspace}
\newcommand{\IDF}{\textsf{IDF}\xspace}
\newcommand{\indices}{\textit{Idx}\xspace}
\newcommand{\BasisExp}{\textsf{BasisExp}\xspace}
\newcommand{\SIMD}{\textsf{SIMD}\xspace}
\newcommand{\Parall}{\textsf{Paral}\xspace}
\newcommand{\DimDecomp}{\textsf{DimDecomp}\xspace}

\newcommand{\maxlen}{\textit{m}\xspace}
\newcommand{\len}{\textsf{len}\xspace}
\newcommand{\packlen}{\textit{u}\xspace}
\newcommand{\numvocab}{\textit{v}\xspace}
\newcommand{\numslot}{\textit{s}\xspace}
\newcommand{\numdoc}{\textsf{num\_doc}\xspace}
\newcommand{\paral}{\textit{h}\xspace}

\newcommand{\itk}{_{i=0}^{K-1}\xspace}
\newcommand{\ktk}{_{k=0}^{K-1}\xspace}


%Additional Algorithms
\newcommand{\Indicator}{\textsf{Indicator}\xspace}
% \newcommand{\ohebasis}{\textsf{OHEbasis}\xspace}
\newcommand{\ohe}{\textit{OHE}\xspace}
\newcommand{\decomp}{\textsf{Decomp}\xspace}
\newcommand{\code}{\textsf{Code}\xspace}
\newcommand{\precision}{\textsf{Precision}\xspace}
\newcommand{\EIF}{\textsf{EEF}\xspace}
\newcommand{\EvalSine}{\textsf{EvalSine}\xspace}


% norm / canonical norm
\newcommand{\Norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\canInfNorm}[1]{\left\Vert #1 \right\Vert_{\infty}^{\textsf{can}}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil {#1} \rceil}
\newcommand{\brac}[1]{\langle {#1} \rangle}
\newcommand{\plain}[1]{\Bar{#1}}
\newcommand{\abs}[1]{| {#1} |}
\newcommand{\cost}[1]{cost_{#1}}


\newcommand{\iter}{\textit{iter}\xspace}
\newcommand{\rownum}{\textit{n_r}\xspace}
\newcommand{\subsize}{\textit{u}\xspace}
\newcommand{\multiplier}{\textit{v}\xspace}
\newcommand{\rounds}{\textit{d}\xspace}


% \newcommand{\colmask}{\plain{m}_{col}\xspace}
% \newcommand{\rowmask}{\plain{m}_{row}\xspace}
\newcommand{\colmask}{\plain{c}\xspace}
\newcommand{\rowmask}{\plain{r}\xspace}
\newcommand{\skewmask}{\plain{s}\xspace}
\newcommand{\rankvec}{\Vec{ct}_{rk}\xspace}
% \newcommand{\vctr}{\Vec{ct}_{comp}\xspace}
\newcommand{\cm}{\Vec{ct}_{B}\xspace}
\newcommand{\CM}{\Vec{C}_{B}\xspace}
\newcommand{\tb}{\Vec{ct}_{tb}\xspace}
\newcommand{\TB}{\Vec{C}_{tb}\xspace}
\newcommand{\targetvec}{\plain{o}\xspace}
\newcommand{\cmk}{\Vec{ct}_{B,k}\xspace}
\newcommand{\tbi}{\Vec{ct}_{tb,i}\xspace}
\newcommand{\crank}{\Vec{ct}_{rk}\xspace}
\newcommand{\crankrc}{\Vec{ct}_{rk,rc}\xspace}
\newcommand{\crankt}{\Vec{ct}_{rk,t}\xspace}
\newcommand{\corder}{\Vec{ct}_{rm}\xspace}


\newcommand{\costrotsum}{C_{RS}\xspace}
\newcommand{\costeif}{C_{EEF}\xspace}
\newcommand{\costeift}{C_{eif,2}\xspace}
\newcommand{\costcomp}{C_{ESF}\xspace}


% algorithm indent
\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
  \begingroup
  \setlength{\itemindent}{\myindent}
  \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Coloring for Editing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}
\newtheorem*{proposition*}{Proposition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}

% \declaretheorem[name=Assumption, sibling=assumption,style=plain]{assum}
% \declaretheorem[name=Theorem, sibling=theorem,style=plain]{thm}
% \declaretheorem[name=Proposition, sibling=proposition,style=plain]{prop}



\usepackage{bm}
% Vectors (bold)
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}

% Bar Notation
\def\bA{{\bar{A}}}
\def\bB{{\bar{B}}}
\def\bC{{\bar{C}}}
\def\bD{{\bar{D}}}
\def\bE{{\bar{E}}}
\def\bF{{\bar{F}}}
\def\bG{{\bar{G}}}
\def\bH{{\bar{H}}}
\def\bI{{\bar{I}}}
\def\bJ{{\bar{J}}}
\def\bK{{\bar{K}}}
\def\bL{{\bar{L}}}
\def\bM{{\bar{M}}}
\def\bN{{\bar{N}}}
\def\bO{{\bar{O}}}
\def\bP{{\bar{P}}}
\def\bQ{{\bar{Q}}}
\def\bR{{\bar{R}}}
\def\bS{{\bar{S}}}
\def\bT{{\bar{T}}}
\def\bU{{\bar{U}}}
\def\bV{{\bar{V}}}
\def\bW{{\bar{W}}}
\def\bX{{\bar{X}}}
\def\bY{{\bar{Y}}}
\def\bZ{{\bar{Z}}}


\def\ba{{\bar{a}}}
\def\bb{{\bar{b}}}
\def\bc{{\bar{c}}}
\def\bd{{\bar{d}}}
\def\be{{\bar{e}}}
% \def\bf{{\bar{f}}}
\def\bg{{\bar{g}}}
\def\bh{{\bar{h}}}
\def\bi{{\bar{i}}}
\def\bj{{\bar{j}}}
\def\bk{{\bar{k}}}
\def\bl{{\bar{l}}}
% \def\bm{{\bar{m}}}
\def\bn{{\bar{n}}}
\def\bo{{\bar{o}}}
\def\bp{{\bar{p}}}
\def\bq{{\bar{q}}}
\def\br{{\bar{r}}}
\def\bs{{\bar{s}}}
\def\bt{{\bar{t}}}
\def\bu{{\bar{u}}}
\def\bv{{\bar{v}}}
\def\bw{{\bar{w}}}
\def\bx{{\bar{x}}}
\def\by{{\bar{y}}}
\def\bz{{\bar{z}}}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}
% \newtheorem{proposition}{Proposition}


% %tikz
% \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
% \tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
% \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=white!30, font=\large]
% \tikzstyle{head} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=white, fill=white!30, draw opacity=0, fill opacity=0, text opacity=1]
% \tikzstyle{party} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=white, fill=white!30, draw opacity=0, fill opacity=0, text opacity=1, font=\large]

% \tikzstyle{arrow} = [thick,->,>=stealth, font=\small]
% \tikzstyle{line} = [thick,-,>=stealth, font=\small]



